Declarative Combinatorics: Boolean Functions, Circuit Synthesis and BDDs in Haskell

We describe Haskell implementations of interesting combinatorial generation algorithms with focus on boolean functions and logic circuit representations. First, a complete exact combinational logic circuit synthesizer is described as a combination of catamorphisms and anamorphisms. Using pairing and unpairing functions on natural number representations of truth tables, we derive an encoding for Binary Decision Diagrams (BDDs) with the unique property that its boolean evaluation faithfully mimics its structural conversion to a a natural number through recursive application of a matching pairing function. We then use this result to derive ranking and unranking functions for BDDs and reduced BDDs. Finally, a generalization of the encoding techniques to Multi-Terminal BDDs is provided. The paper is organized as a self-contained literate Haskell program, available at http://logic.csci.unt.edu/tarau/research/2008/fBDD.zip . Keywords: exact combinational logic synthesis, binary decision diagrams, encodings of boolean functions, pairing/unpairing functions, ranking/unranking functions for BDDs and MTBDDs, declarative combinatorics in Haskell

==> TOOLS/spheader.tex <==
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{subfig}
\usepackage{url}
\usepackage{verbatim} 
\usepackage{listings}
\lstloadlanguages{Prolog}
\lstnewenvironment{code}
    {\lstset{}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    \lstset{
      basicstyle=\small\ttfamily,
      flexiblecolumns=false,
      basewidth={0.5em,0.45em},
      literate={+}{{$+$}}1 {*}{{$*$}}1 {=}{{$=$}}1
               {>}{{$>$}}1 {<}{{$<$}}1
               {<-}{{$\leftarrow$}}2
               {|}{{$\mid$}}1               
    }
\newtheorem{prop}{Proposition}
\newtheorem{df}{Definition}

\def \bscale1 {1.00}
\def \bscale {0.20}
\def \hscale {0.20}

% \FIG{Label}{Title}{PNG}
\newcommand{\FIG}[3]{
\begin{figure}[htbp]
\centering
\scalebox{\bscale1}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#3.png}}
\caption{#2}
\label{#1}
\end{figure}
}

% \HFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\HFIGS}[6]{
\begin{figure}[htbp]
  \centering
  \subfloat[#3]{
    {\scalebox{\hscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]
    {./figs/#5.png}}}} 
  \subfloat[#4]{
    {\scalebox{\hscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]
    {./figs/#6.png}}}}
  \caption{#2}
  \label{#1}
\end{figure}
}

% \VFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\VFIGS}[6]{
\begin{figure}[htbp]
  \begin{center}
    {\scalebox{\bscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#5.png}}}
    {\scalebox{\bscale}{\includegraphics*[bb=0pt 0pt 800pt 800pt]{./figs/#6.png}}}
  \caption{#2: {\em #3} and {\em #4}}
  \label{#1}
  \end{center}
\end{figure}
}

